Phase Retrieval using Alternating Minimization

Phase retrieval problems involve solving linear equations, but with missing sign (or phase, for complex numbers) information. More than four decades after it was first proposed, the seminal error reduction algorithm of (Gerchberg and Saxton 1972) and (Fienup 1982) is still the popular choice for solving many variants of this problem. The algorithm is based on alternating minimization; i.e. it alternates between estimating the missing phase information, and the candidate solution. Despite its wide usage in practice, no global convergence guarantees for this algorithm are known. In this paper, we show that a (resampling) variant of this approach converges geometrically to the solution of one such problem -- finding a vector $\mathbf{x}$ from $\mathbf{y},\mathbf{A}$, where $\mathbf{y} = \left|\mathbf{A}^{\top}\mathbf{x}\right|$ and $|\mathbf{z}|$ denotes a vector of element-wise magnitudes of $\mathbf{z}$ -- under the assumption that $\mathbf{A}$ is Gaussian. Empirically, we demonstrate that alternating minimization performs similar to recently proposed convex techniques for this problem (which are based on "lifting" to a convex matrix problem) in sample complexity and robustness to noise. However, it is much more efficient and can scale to large problems. Analytically, for a resampling version of alternating minimization, we show geometric convergence to the solution, and sample complexity that is off by log factors from obvious lower bounds. We also establish close to optimal scaling for the case when the unknown vector is sparse. Our work represents the first theoretical guarantee for alternating minimization (albeit with resampling) for any variant of phase retrieval problems in the non-convex setting.

==> convergence.tex <==
\begin{lemma}\label{lem:convergence}
  Suppose in iteration $t$ of Algorithm \ref{algo:phasesensing-nonsparse}, we have $\dist{\vecfont{x^t}}{\vecfont{x^*}} < c_1$. Then, there exists a constant
  $\widehat{c}$ such that if the number of columns of $\mat{A^t}$ is greater than $\widehat{c}n$ then with probability more than $1 - \exp\left(-n\right)$ we have:
\begin{align*}
  \dist{\vecfont{x^{t+1}}}{\vecfont{x^*}} < \frac{2}{3} \dist{\vecfont{x^t}}{\vecfont{x^*}}.
\end{align*}
\end{lemma}
\begin{proof}
For simplicity of notation in the proof of the lemma, we will use $\mat{A}$ for $\mat{A^{t+1}}$, $\mat{C}$ for $\mat{C^{t+1}}$, $\vecfont{x}$ for $\vecfont{x^t}$, $\vecfont{\xplus}$ for
$\vecfont{x^{t+1}}$ and $\vecfont{y}$ for $\vecfont{y^{t+1}}$.
We have:
\begin{align*}
  \vecfont{\xplus} &= \argmin_{\vecfont{\widetilde{x}}\in \rn} \twonorm{\mat{A}^T \vecfont{\widetilde{x}} - \mat{C}\vecfont{y}} \\
  &= \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\mat{C}\vecfont{y} \\
  &= \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\mat{D}\mat{A}^T\vecfont{x^*},  
\end{align*}
where $D$ is a diagonal matrix with $d_{ll} \eqdef \phase{\vecfont{a_l}^T\vecfont{x}\cdot \conj{\vecfont{a_l}^T\vecfont{x^*}}}$.
Fix a unit vector $z$ such that $z \perp x^*$. Wlog, assume the following:
\begin{enumerate}
  \item	$\vecfont{x^*} = \vecfont{e_1}$,
  \item	$\vecfont{x} = \alpha \vecfont{e_1} + \sqrt{1-\alpha^2} \vecfont{e_2}$ where $\alpha\in \reals$ and $\alpha \geq 0$, and
  \item	$\vecfont{z} = \beta \vecfont{e_2} + \sqrt{1-\abs{\beta}^2} \vecfont{e_3}$ for some $\beta \in \complex$.
\end{enumerate}
We will first show the following:
\begin{itemize}
  \item	$\abs{\vecfont{x^*}^T \vecfont{\xplus}} \geq 1 - c \sqrt{1-\alpha^2}$ and,
  \item	$\abs{\vecfont{z}^T \vecfont{\xplus}} \leq \left(\frac{\beta}{2}+\delta\right) \sqrt{1-\alpha^2}$.
\end{itemize}
Using union bound, the second result above can be generalized for all vectors $\vecfont{z}$ that are orthogonal to $\vecfont{x^*}$.
We will then use the above results to prove the lemma. We begin by writing $\vecfont{\xplus}$ in a convenient form:
\begin{align*}
  \vecfont{\xplus} &= \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\mat{D}\mat{A}^T\vecfont{e_1} \\
	&= \vecfont{e_1} + \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}.
\end{align*}
We now calculate the following quantities:
\begin{align}
  \abs{\vecfont{e_1}^T \vecfont{\xplus}} &= \abs{1 + \vecfont{e_1}^T \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber\\
	&\geq 1 - \abs{\vecfont{e_1}^T \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber \\
	&\geq 1 - \frac{1}{2m}\twonorm{\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1}} \twonorm{\mat{A}} \twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}},
		\label{eqn:e1Txplus} \\
  \abs{\vecfont{e_2}^T \vecfont{\xplus}} &= \abs{\vecfont{e_2}^T \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber\\
	&\leq \frac{1}{2m}\abs{\vecfont{e_2}^T \left(\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}\right)\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	  + \frac{1}{2m}\abs{\vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber \\
	&\leq \frac{1}{2m}\twonorm{\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}}\twonorm{\mat{A}}\twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	  + \frac{1}{2m}\abs{\vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}, \mbox{ and} \label{eqn:e2Txplus} \\
  \abs{\vecfont{e_3}^T \vecfont{\xplus}} &= \abs{\vecfont{e_3}^T \left(\mat{A}\mat{A}^T\right)^{-1}\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber\\
	&\leq \frac{1}{2m}\abs{\vecfont{e_3}^T \left(\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}\right)\mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	  + \frac{1}{2m}\abs{\vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \nonumber \\
	&\leq \frac{1}{2m}\twonorm{\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}}\twonorm{\mat{A}}\twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	  + \frac{1}{2m}\abs{\vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}. \label{eqn:e3Txplus}
\end{align}
In order to bound \eqref{eqn:e1Txplus}-\eqref{eqn:e3Txplus}, we bound the following quantities:
\begin{enumerate}
  \item	$\twonorm{\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}}$ (Lemma \ref{lem:AATinv})
  \item	$\twonorm{\mat{A}}$ (Lemma \ref{lem:A})
  \item	$\twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}$ (Lemma \ref{lem:e1err})
  \item	$\abs{\vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}$ (Lemma \ref{lem:e2err})
  \item	$\abs{\vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}$ (Lemma \ref{lem:e3err})
\end{enumerate}
\end{proof}

\begin{lemma}\label{lem:AATinv}
  Suppose $A$ is an $m\times n$ matrix with independent standard complex Gaussian entries where $m > \frac{n}{\delta^2}$.
Then, with probability greater than $1 - e^{-n}$, we have the following:
\begin{align*}
  \twonorm{\left(\frac{1}{2m}\mat{A}\mat{A}^T\right)^{-1} - \mat{I}} \leq \delta.
\end{align*}
\end{lemma}

\begin{lemma}\label{lem:A}
  Suppose $A$ is an $m\times n$ matrix with independent standard complex Gaussian entries where $m > \frac{n}{\delta^2}$.
Then, with probability greater than $1 - e^{-n}$, we have the following:
\begin{align*}
  \frac{1}{\sqrt{2m}}\twonorm{\mat{A}} \leq 1+\delta.
\end{align*}  
\end{lemma}

\begin{lemma}\label{lem:e1err}
  Assume the hypothesis of Lemma \ref{lem:convergence}. Then, there exists an absolute numerical constant $c$ such that:
\begin{align*}
  \twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \leq c \sqrt{m}\sqrt{1-\alpha^2},
\end{align*}
with probability greater than $1-e^{-n}$.
\end{lemma}
\begin{proof}
  We have:
\begin{align*}
  \twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}^2
	= \sum_{l=1}^m \abs{a_{1l}}^2 \abs{\phase{\left(\alpha \conj{a}_{1l}+\sqrt{1-\alpha^2} \conj{a}_{2l}\right) a_{1l}}-1}^2.
\end{align*}
Define the random variable $U_l$ as follows:
\begin{align*}
  U_l \eqdef \abs{a_{1l}}^2 \abs{\phase{\left(\alpha \conj{a}_{1l}+\sqrt{1-\alpha^2} \conj{a}_{2l}\right) a_{1l}}-1}^2.
\end{align*}
We will first calculate $\prob{U_l > t}$ to:
\begin{enumerate}
  \item	calculate $\expec{U_l}$ and,
  \item	show that $U_l$ is a subexponential random variable and use that fact to derive concentration bounds.
\end{enumerate}
We have:
\begin{align*}
  \prob{U_l > t} = \int_{\frac{\sqrt{t}}{2}}^{\infty} p_{\abs{a_{1l}}}(s) \prob{W_l > \frac{\sqrt{t}}{s} \middle| \abs{a_{1l}} = s} ds,
\end{align*}
where $W_l \eqdef \abs{\phase{\left(\alpha \conj{a}_{1l}+\sqrt{1-\alpha^2} \conj{a}_{2l}\right) a_{1l}}-1}$.
\begin{align*}
  \prob{W_l > \frac{\sqrt{t}}{s} \middle| \abs{a_{1l}} = s}
	&= \prob{\abs{\phase{\left(\alpha \conj{a}_{1l}+\sqrt{1-\alpha^2} \conj{a}_{2l}\right) a_{1l}}-1} > \frac{\sqrt{t}}{s}
		\middle| \abs{a_{1l}} = s} \\
	&= \prob{\abs{\phase{1+\frac{\sqrt{1-\alpha^2} \conj{a}_{2l}}{\alpha \conj{a}_{1l}}}-1} > \frac{\sqrt{t}}{s}
		\middle| \abs{a_{1l}} = s} \\
	&\stackrel{(\zeta_1)}{\leq} \prob{\frac{\sqrt{1-\alpha^2} \abs{a_{2l}}}{\alpha \abs{a_{2l}}} > \frac{c\sqrt{t}}{s}
		\middle| \abs{a_{1l}} = s} \\
	&= \prob{\abs{a_{2l}} > \frac{c\alpha\sqrt{t}}{\sqrt{1-\alpha^2}}} \\
	&\stackrel{(\zeta_2)}{\leq} \exp\left(1-\frac{c\alpha^2 t}{1-\alpha^2}\right),
\end{align*}
where $(\zeta_1)$ follows from Lemma \ref{lem:phase-absvalue} and $(\zeta_2)$ follows from the fact that
$a_{2l}$ is a sub-gaussian random variable.
So we have:
\begin{align}
  \prob{U_l > t} &\leq \int_{\frac{\sqrt{t}}{2}}^{\infty} \exp\left(1-\frac{c\alpha^2 t}{1-\alpha^2}\right) ds \nonumber\\
	&= \exp\left(1-\frac{c\alpha^2 t}{1-\alpha^2}\right) \int_{\frac{\sqrt{t}}{2}}^{\infty} s e^{-\frac{s^2}{2}} ds
	 = \exp\left(1 - \frac{ct}{1-\alpha^2}\right). \label{eqn:Ultailbound}
\end{align}
Using this, we have the following bound on the expected value of $U_l$:
\begin{align}
  \expec{U_l} &= \int_0^{\infty} \prob{U_l > t} dt \nonumber\\
	&\leq \int_0^{\infty} \exp\left(1 - \frac{ct}{1-\alpha^2}\right) dt 
	\leq c\left(1-\alpha^2\right).
\end{align}
From \eqref{eqn:Ultailbound}, we see that $U_l$ is a subexponential random variable with parameter $c\left(1-\alpha^2\right)$.
Using Proposition 5.16 from \cite{Vershynin10}, we obtain:
\begin{align*}
  \prob{\abs{\sum_{l=1}^m U_l - \expec{U_l}} > \delta m \left(1-\alpha^2\right)}
	&\leq 2 \exp\left(-\min\left(\frac{c\delta^2 m^2 \left(1-\alpha^2\right)^2}{\left(1-\alpha^2\right)^2m},
		\frac{c\delta m \left(1-\alpha^2\right)}{1-\alpha^2}\right)\right) \\
	&\leq 2 \exp\left(-c\delta^2 m\right) \leq \exp\left(-n\right).
\end{align*}
So, with probability greater than $1 - \exp(-n)$, we have:
\begin{align*}
  \twonorm{\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	&= \sqrt{\sum_{l=1}^m U_l}
	 \leq c\sqrt{m}\sqrt{(1-\alpha^2)}.
\end{align*}
This proves the lemma.
\end{proof}

\begin{lemma}\label{lem:e2err}
  Assume the hypothesis of Lemma \ref{lem:convergence}. Then,
\begin{align*}
  \abs{\vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \leq (1+\delta) m \sqrt{1-\alpha^2},
\end{align*}
with probability greater than $1-e^{-n}$.
\end{lemma}
\begin{proof}
We have:
\begin{align*}
  \vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}
	&= \sum_{l=1}^m \conj{a}_{1l} a_{2l} \left(\phase{\left(\alpha \conj{a}_{1l}+\sqrt{1-\alpha^2} \conj{a}_{2l}\right) a_{1l}}-1\right) \\
	&= \sum_{l=1}^m \abs{a_{1l}} a'_{2l} \left(\phase{\alpha \abs{a_{1l}}+\sqrt{1-\alpha^2} \conj{a'_{2l}}}-1\right),
\end{align*}
where $a'_{2l} \eqdef a_{2l}\phase{\conj{a}_{1l}}$ is identically distributed to $a_{2l}$ and is independent of
$\abs{a_{1l}}$. Define the random variable $U_l$ as:
\begin{align*}
  U_l \eqdef \abs{a_{1l}} a'_{2l} \left(\phase{1+\frac{\sqrt{1-\alpha^2} \conj{a'_{2l}}}{\alpha \abs{a_{1l}}}}-1\right).
\end{align*}
Similar to Lemma \ref{lem:e1err}, we will calculate $\prob{U_l > t}$ to show that $U_l$ is subexponential and use it to derive concentration
bounds. However, using the above estimate to bound $\expec{U_l}$ will result in a weak bound that we will not be able to use.
Lemma \ref{lem:e2err-expected-value-bound} bounds $\expec{U_l}$ using a different technique carefully.
\begin{align*}
  \prob{\abs{U_l} > t} &\leq \prob{ \abs{a_{1l}} \abs{a'_{2l}} \frac{c\sqrt{1-\alpha^2} \abs{a'_{2l}}}{\alpha \abs{a_{1l}}} > t} \\
	&= \prob{ \abs{a'_{2l}}^2  > \frac{c\alpha t}{\sqrt{1-\alpha^2}}}
	\leq \exp\left(1-\frac{c\alpha t}{\sqrt{1-\alpha^2}}\right),
\end{align*}
where the last step follows from the fact that $a'_{2l}$ is a subgaussian random variable and hence $\abs{a'_{2l}}^2$ is
a subexponential random variable. Using Proposition 5.16 from \cite{Vershynin10}, we obtain:
\begin{align*}
  \prob{\abs{\sum_{l=1}^m U_l - \expec{U_l}} > \delta m \sqrt{1-\alpha^2}}
	&\leq 2 \exp\left(-\min\left(\frac{c\delta^2 m^2 \left(1-\alpha^2\right)}{\left(1-\alpha^2\right)m},
		\frac{c\delta m \sqrt{1-\alpha^2}}{\sqrt{1-\alpha^2}}\right)\right) \\
	&\leq 2 \exp\left(-c\delta^2 m\right) \leq \exp\left(-n\right).
\end{align*}
Using Lemma \ref{lem:e2err-expected-value-bound}, we obtain:
\begin{align*}
  \abs{\vecfont{e_2}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	&= \abs{\sum_{l=1}^m U_l}
	\leq \left(1+\delta\right) m \sqrt{1-\alpha^2},
\end{align*}
with probability greater than $1 - \exp(-n)$. This proves the lemma.
\end{proof}

\begin{lemma}\label{lem:e2err-expected-value-bound}
  Let $w_1$ and $w_2$ be two independent standard complex gaussian random variables. Let
\begin{align*}
  U = \abs{w_1} w_2 \left(\phase{1+\frac{\sqrt{1-\alpha^2} \conj{w_2}}{\alpha \abs{w_1}}}-1\right).
\end{align*}
Fix $\delta > 0$. Then, there exists an absolute numerical constant $\gamma > 0$ such that if $\sqrt{1-\alpha^2} < \gamma$,
then:
\begin{align*}
  \expec{U} \leq (1+\delta) \sqrt{1-\alpha^2}.
\end{align*}
\end{lemma}
\begin{proof}
Let $w_2 = \abs{w_2} e^{i\theta}$. Then $\abs{w_1}, \abs{w_2}$ and $\theta$ are all independent random variables. $\theta$ is a uniform random
variable over $[-\pi,\pi]$ and $\abs{w_1}$ and $\abs{w_2}$ are identically distributed with probability distribution function:
\begin{align*}
  p(x) = x \exp\left(-\frac{x^2}{2}\right) \mathds{1}_{\{x \geq 0\}}.
\end{align*}
We have:
\begin{align*}
  \expec{U} &= \expec{\abs{w_1} \abs{w_2} e^{i\theta} \left(\phase{1+\frac{\sqrt{1-\alpha^2} \abs{w_2}e^{-i\theta}}{\alpha \abs{w_1}}}-1\right)} \\
	&= \expec{\abs{w_1} \abs{w_2} \expec{e^{i\theta} \left(\phase{1+\frac{\sqrt{1-\alpha^2} \abs{w_2}e^{-i\theta}}{\alpha \abs{w_1}}}-1\right)}\middle| \abs{w_1}, \abs{w_2}} \\
\end{align*}
Let $\beta \eqdef \frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}$. We will first calculate $\expec{e^{i\theta} \phase{1+\beta e^{-i\theta}}\middle| \abs{w_1}, \abs{w_2}}$.
Note that the above expectation is taken only over the randomness in $\theta$.
For simplicity of notation, we will drop the conditioning variables, and calculate the above expectation in terms of $\beta$.
\begin{align*}
  e^{i\theta} \phase{1+\beta e^{-i\theta}} &= \left(\cos \theta + i \sin \theta\right) \frac{1+\beta \cos \theta - i \beta \sin \theta}{\left[\left(1+\beta\cos\theta\right)^2 + \beta^2 \sin^2\theta\right]^{\frac{1}{2}}} \\
	&= \frac{\cos \theta + \beta + i \sin \theta}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{1}{2}}}.
\end{align*}
We will first calculate the imaginary part of the above expectation:
\begin{align}
  \imag{\expec{e^{i\theta} \phase{1+\beta e^{-i\theta}}}} = \expec{\frac{\sin \theta}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{1}{2}}}} = 0, \label{eqn:e2err-expec-imag}
\end{align}
where the last step follows because we are taking the expectation of an odd function. Focusing on the real part, we let:
\begin{align*}
  F(\beta) &\eqdef \expec{\frac{\cos \theta + \beta}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{1}{2}}}} \\
	&= \frac{1}{2\pi} \int_{-\pi}^\pi \frac{\cos \theta + \beta}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{1}{2}}} d\theta.
\end{align*}
Note that $F(\beta):\reals \rightarrow \reals$ and $F(0)=0$. We will show that there is a small absolute numerical constant $\gamma$ (depending on $\delta$) such that:
\begin{align}\label{eqn:e2err-expec-smallbetabound}
  0 < \beta < \gamma \Rightarrow \abs{F(\beta)} \leq (\frac{1}{2}+\delta) \beta.
\end{align}
We show this by calculating $F'(0)$ and using the continuity of $F'(\beta)$ at $\beta = 0$.
We first calculate $F'(\beta)$ as follows:
\begin{align*}
  F'(\beta) &= \frac{1}{2\pi} \int_{-\pi}^\pi \frac{1}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{1}{2}}} -
  \frac{\left(\cos \theta + \beta\right)\left(\beta+\cos \theta\right)}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{3}{2}}} d\theta \\
	&= \frac{1}{2\pi} \int_{-\pi}^\pi \frac{\sin^2 \theta}{\left(1+\beta^2+2\beta\cos\theta\right)^{\frac{3}{2}}} d\theta
\end{align*}
From the above, we see that $F'(0)=\frac{1}{2}$ and \eqref{eqn:e2err-expec-smallbetabound} then follows from the continuity of $F'(\beta)$ at $\beta=0$.
Getting back to the expected value of $U$, we have:
\begin{align}
  \abs{\expec{U}} &= \left|\expec{\abs{w_1} \abs{w_2} F\left(\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\right) \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}< \gamma\right\}}} \right.\nonumber\\
	&\;\;\;\;\;\left.+ \expec{\abs{w_1} \abs{w_2} F\left(\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\right) \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}}\right|\nonumber\\
	&= \left|\expec{\abs{w_1} \abs{w_2} F\left(\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\right) \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}< \gamma\right\}}} \right|\nonumber\\
	&\;\;\;\;\;+ \left|\expec{\abs{w_1} \abs{w_2} F\left(\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\right) \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}}\right| \nonumber\\
	&\stackrel{(\zeta_1)}{\leq} \left(\frac{1}{2}+\delta\right)\expec{\abs{w_1} \abs{w_2} \frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}}
	+ \expec{\abs{w_1} \abs{w_2} \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}},\nonumber\\
	&= \left(\frac{1}{2}+\delta\right)\left(\frac{\sqrt{1-\alpha^2}}{\alpha}\right)\expec{\abs{w_2}^2}
	+ \expec{\abs{w_1} \abs{w_2} \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}},\nonumber\\
	&\stackrel{(\zeta_2)}{=} \left(1+2\delta\right)\left(\frac{\sqrt{1-\alpha^2}}{\alpha}\right)
	+ \expec{\abs{w_1} \abs{w_2} \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}},\label{eqn:e2err-expec-betabound}
\end{align}
where $(\zeta_1)$ follows from \eqref{eqn:e2err-expec-smallbetabound} and the fact that $\abs{F(\beta)} \leq 1$ for every $\beta$ and
$(\zeta_2)$ follows from the fact that $\expec{\abs{z_2}^2}=2$.
We will now bound the second term in the above inequality. We start with the following integral:
\begin{align}
  \int_t^{\infty} s^2 e^{-\frac{s^2}{2}} ds &= -\int_t^{\infty} s d\left(e^{-\frac{s^2}{2}}\right) \nonumber \\
	&= te^{-\frac{t^2}{2}} + \int_t^{\infty} e^{-\frac{s^2}{2}} ds
	\leq (t+e) e^{-\frac{t^2}{c}},\label{eqn:e2err-expec-intbound}
\end{align}
where $c$ is some constant. The last step follows from standard bounds on the tail probabilities of gaussian random variables.
We now bound the second term of \eqref{eqn:e2err-expec-betabound} as follows:
\begin{align*}
  \expec{\abs{w_1} \abs{w_2} \mathds{1}_{\left\{\frac{\sqrt{1-\alpha^2} \abs{w_2}}{\alpha \abs{w_1}}\geq \gamma\right\}}}
	&= \int_0^{\infty} t^2 e^{-\frac{t^2}{2}} \int_{\frac{\alpha t}{\sqrt{1-\alpha^2}}}^{\infty} s^2 e^{-\frac{s^2}{2}} ds dt \\
	&\stackrel{(\zeta_1)}{\leq} \int_0^{\infty} t^2 e^{-\frac{t^2}{2}} \left(\frac{\alpha t}{\sqrt{1-\alpha^2}}+e\right) e^{-\frac{\alpha^2 t^2}{c\left(1-\alpha^2\right)}} dt \\
	&\leq \int_0^{\infty} \left(\frac{\alpha t^3}{\sqrt{1-\alpha^2}}+et^2\right) e^{-\frac{t^2}{c\left(1-\alpha^2\right)}} dt \\
	&= \frac{\alpha}{\sqrt{1-\alpha^2}}\int_0^{\infty} t^3 e^{-\frac{t^2}{c\left(1-\alpha^2\right)}} dt + e\int_0^{\infty} t^2 e^{-\frac{t^2}{c\left(1-\alpha^2\right)}} dt \\
	&\stackrel{(\zeta_2)}{\leq} c \left(1-\alpha^2\right)^{\frac{3}{2}}
	\stackrel{(\zeta_3)}{\leq} \delta \sqrt{1-\alpha^2}
\end{align*}
where $(\zeta_1)$ follows from \eqref{eqn:e2err-expec-intbound}, $(\zeta_2)$ follows from the formulae for second and third absolute moments of gaussian random variables
and $(\zeta_3)$ follows from the fact that $1-\alpha^2 < \delta$. Plugging the above inequality in \eqref{eqn:e2err-expec-betabound}, we obtain:
\begin{align*}
  \abs{\expec{U}} \leq \left(1+2\delta\right)\left(\frac{\sqrt{1-\alpha^2}}{\alpha}\right) + \delta \sqrt{1-\alpha^2}
	\leq \left(1+4\delta\right)\sqrt{1-\alpha^2},
\end{align*}
where we used the fact that $\alpha \geq 1 - \frac{\delta}{2}$. This proves the lemma.
\end{proof}


\begin{lemma}\label{lem:e3err}
  Assume the hypothesis of Lemma \ref{lem:convergence}. Then,
\begin{align*}
  \abs{\vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}} \leq \delta m \sqrt{1-\alpha^2},
\end{align*}
with probability greater than $1-e^{-n}$.
\end{lemma}
\begin{proof}
The proof of this lemma is very similar to that of Lemma \ref{lem:e2err}.
We have:
\begin{align*}
  \vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}
	&= \sum_{l=1}^m \conj{a}_{1l} a_{3l} \left(\phase{\left(\alpha \conj{a}_{1l}+\conj{a}_{2l}\sqrt{1-\alpha^2} \conj{a}_{3l}\right) a_{1l}}-1\right) \\
	&= \sum_{l=1}^m \abs{a_{1l}} a'_{3l} \left(\phase{\alpha \abs{a_{1l}}+\conj{a'_{2l}}\sqrt{1-\alpha^2} }-1\right),
\end{align*}
where $a'_{3l} \eqdef a_{3l}\phase{\conj{a}_{1l}}$ is identically distributed to $a_{3l}$ and is independent of
$\abs{a_{1l}}$ and $a'_{2l}$. Define the random variable $U_l$ as:
\begin{align*}
  U_l \eqdef \abs{a_{1l}} a'_{3l} \left(\phase{1+\frac{\conj{a'_{2l}}\sqrt{1-\alpha^2} }{\alpha \abs{a_{1l}}}}-1\right).
\end{align*}
Since $a'_{3l}$ has mean zero and is independent of everything else, we have:
\begin{align*}
  \expec{U_l} = 0.
\end{align*}
Similar to Lemma \ref{lem:e2err}, we will calculate $\prob{U_l > t}$ to show that $U_l$ is subexponential and use it to derive concentration
bounds.
\begin{align*}
  \prob{\abs{U_l} > t} &\leq \prob{ \abs{a_{1l}} \abs{a'_{3l}} \frac{c\sqrt{1-\alpha^2} \abs{a'_{2l}}}{\alpha \abs{a_{1l}}} > t} \\
	&= \prob{ \abs{a'_{2l}a'_{3l}}  > \frac{c\alpha t}{\sqrt{1-\alpha^2}}}
	\leq \exp\left(1-\frac{c\alpha t}{\sqrt{1-\alpha^2}}\right),
\end{align*}
where the last step follows from the fact that $a'_{2l}$ and $a'_{3l}$ are independent subgaussian random variables and hence $\abs{a'_{2l}a'_{3l}}$ is
a subexponential random variable. Using Proposition 5.16 from \cite{Vershynin10}, we obtain:
\begin{align*}
  \prob{\abs{\sum_{l=1}^m U_l - \expec{U_l}} > \delta m \sqrt{1-\alpha^2}}
	&\leq 2 \exp\left(-\min\left(\frac{c\delta^2 m^2 \left(1-\alpha^2\right)}{\left(1-\alpha^2\right)m},
		\frac{c\delta m \sqrt{1-\alpha^2}}{\sqrt{1-\alpha^2}}\right)\right) \\
	&\leq 2 \exp\left(-c\delta^2 m\right) \leq \exp\left(-n\right).
\end{align*}
Hence, we have:
\begin{align*}
  \abs{\vecfont{e_3}^T \mat{A}\left(\mat{D}-\mat{I}\right)\mat{A}^T\vecfont{e_1}}
	&= \abs{\sum_{l=1}^m U_l}
	\leq \delta m \sqrt{1-\alpha^2},
\end{align*}
with probability greater than $1 - \exp(-n)$. This proves the lemma.
\end{proof}

\begin{lemma}\label{lem:phase-absvalue}
For every $w \in \complex$, we have:
\begin{align*}
  \abs{\phase{1+w}-1} \leq 2 \abs{w}.
\end{align*}
\end{lemma}
\begin{proof}
The proof is straight forward:
\begin{align*}
  \abs{\phase{1+w}-1} \leq \abs{\phase{1+w}-(1+w)} + \abs{w}
	= \abs{1-\abs{1+w}} + \abs{w}
	\leq 2 \abs{w}.
\end{align*}
\end{proof}


==> discussion.tex <==
\section{Conclusion and Discussion}\label{sec:discussion}
In this paper, we present an improved version of the alternating minimization procedure for the phase retrieval problem. We observe that empirically,
it has simiar sample complexity as SDP based methods but is much more efficient than them. Analytically, we show that a natural resampled version of this
algorithm has close to optimal sample complexity. We also extend our algorithm and results for the sparse phase retrieval problem.

In a broader context, alternating minimization is a popular empirical approach for solving a variety of problems. However, there are few theoretical guarantees
regarding its performance. We believe that understanding the performance of alternating minimization procedure and extending its theoretical guarantees
to more problems is important from two points of view:
\begin{enumerate}
  \item	It help us gain insight into designing better settings, such as measurement schemes, and
  \item	It helps us in improving upon the basic algorithm, such as the initialization procedure.
\end{enumerate}
So far, matrix sensing and matrix completion, and now the phase retrieval problem are the only ones with theoretical guanratees
for the alternating minimization procedure. We believe that the techniques of this paper may prove useful in obtaining such guarantees for other problems.
